Sig-Splines: universal approximation and convex calibration of time series generative models

We propose a novel generative model for multivariate discrete-time time series data. Drawing inspiration from the construction of neural spline flows, our algorithm incorporates linear transformations and the signature transform as a seamless substitution for traditional neural networks. This approach enables us to achieve not only the universality property inherent in neural networks but also introduces convexity in the model's parameters.

==> definitions.tex <==
\section{Signatures}
\begin{definition}[Tensor algebra]
    Let $ d\geq 1$. We define the extended tensor algebra over $\mathbb{R}^d$ by 
    \begin{equation*}
        T((\mathbb{R}^d)) \coloneqq \lbrace 
        \mathbf{a} = (a_0, a_1, \dots, a_n, \dots) \ | \ a_n \in (\mathbb{R}^d)^{\otimes n}\rbrace.
    \end{equation*}
Similarly, we define the truncated tensor algebra of order $N\in \mathbb{N}$ and the tensor algebra by $T^{(N)}(\mathbb{R}^d)$ and $T(\mathbb{R}^d)$ respectively, by
\begin{equation*}
    T^{(N)}(\mathbb{R}^d) \coloneqq \lbrace \mathbf{a}=(a_n)_{n=0}^\infty \ | \ a_n \in (\mathbb{R}^d)^{\otimes n} \ \textrm{and} \ a_n = 0 \ \forall n \geq N \rbrace \subset T((\mathbb{R}^d)),
\end{equation*}
\begin{equation*}
    T(\mathbb{R}^d) \coloneqq \bigcup_{n\geq 0} T^{(n)}(\mathbb{R}^d) \subset T((\mathbb{R}^d)).
\end{equation*}
\end{definition}
\begin{remark}
We denote the dual space of $\mathbb{R}^d$ by $(\mathbb{R}^d)^*$ and the tensor algebra of the space $(\mathbb{R}^d)^*$ by $T((\mathbb{R}^d)^*)$.
\end{remark}

The vector space $\R^d$ is spanned by a $d$-dimensional basis $\lbrace e_1, \dots, e_d \rbrace$. We denote by $[d] = \lbrace 1, \dots, d \rbrace$ the set of $d$ letters. $[d]^\star = \cup_{m\geq 0} [d]^{\times m} $ will denote the set of all multi-indices. 

Real-world paths are not sampled continuously in general, but at discrete time stamps. Before we define the signature we shall define the space of sequences. 
\begin{definition}[Sequence space]
    Let $V$ be a space. We call the space 
    \begin{equation*}
        S(V) \coloneqq \lbrace \mathbf{x} = (\mathbf x_1, \dots, \mathbf x_n) \ | \ \mathbf x_i \in V, i=1, \dots, n \ , n \geq 1\rbrace
    \end{equation*}
    the \emph{sequence space of $V$}. 
\end{definition}


\begin{remark}[Truncated signature]
In practice, we work with \emph{truncated} signatures, where the truncated signature of order $L \in \N$ is simply the sequence composed from the first $L$ iterated integrals. The error in performing this truncation decays at rate $\mathcal{O}(1/L!)$ \cite{lyons2007differential}. The \emph{signature of $\mathbf{x}$ truncated at order $L \in \N$} is defined as 
$$ 
\Sig^{(L)}(\mathbf{x}) = \left(1, \left(\Sig_{\mathbf{i}}(\mathbf x)\right)_{\mathbf{i} \in [d]}, \dots, \left(\Sig_{\mathbf{i}}(\mathbf x)\right)_{\mathbf{i} \in [d]^{\times L}}, \mathbf{0}, \mathbf{0}, \dots \right) \in T^{(L)}(\R^d) 
$$
where $\mathbf{0}$ denotes the corresponding tensor filled with zeroes. The number of terms in the truncated signature of a $d$-dimensional process, truncated at order $L$ is 
\begin{equation*}
    f(d, L) \coloneqq \sum_{k = 0}^L d^k = \dfrac{d^{L+1}-1}{d-1} . 
\end{equation*}
\end{remark}


The signature of a path in general does not fully determine the path due to translational invariance (the signature as a collection of iterated integrals is independent of the path's starting point) and invariance under time parametrisation. To obtain the universality approximation theorem of signatures we introduce the space of time-augmented paths with bounded variation starting at zero and denote it by $\Omega_0([0, 1]; \R^d)\coloneqq \lbrace \rbrace $. Note that any sequence can be embedded into this space by adding time stamps to the sequence and a basepoint. We denote the embedding function by $\Gamma: S(\R^d) \to S(\R^{1+d})$ and which is defined for $\mathbf{x} \in S(\R^d)$ as 
\begin{equation*}
    \Gamma(\mathbf{x}) = 
    \left(\begin{array}{cccc}
        t_0 & t_1 & \dots & t_n\\
        \mathbf{0} & \mathbf{x}_1 & \dots & \mathbf{x}_n
    \end{array}\right) . 
\end{equation*} 

we define two fundamental sequence augmentations which remove both invariance properties of signatures. 

\begin{definition}[Basepoint augmentatino]
    We call the function $\phi: S(\R^d) \to S(\R^d)$ defined as 
    \begin{equation*}
        \phi: (\mathbf{x}_1, \dots, \mathbf{x}_n) \mapsto 
        (\mathbf{0}, \mathbf{x}_1, \dots, \mathbf{x}_n)
    \end{equation*}
    \emph{basepoint augmentation}. 
\end{definition}
\begin{definition}
    We call the function $\psi: S(\R^d) \to S(\R^{1+d})$ defined as 
    \begin{equation*}
    \psi: (\mathbf{x}_1, \dots, \mathbf{x}_n) \mapsto 
    \left(\begin{array}{ccc}
        t_1 & \dots & t_n\\
        \mathbf{x}_1 & \dots & \mathbf{x}_n
    \end{array}\right)
    \end{equation*}
    \emph{time augmentation}. 
\end{definition}
 
\begin{definition}{Mask augmentation}    
    Denote the space of $\R^d$-valued sequences of length greater than $n \in \mathbb{N}$ by $S(\R^d, n)$. The function $m: S(\R^d, 2) \times [d] \to S(\R^d, 2)$ defined for $i =1$ as 
    \begin{equation*}
        m(\mathbf{x}, i)  = \left(\mathbf{x}_1, \dots, \mathbf{x}_{n-1} \right)
    \end{equation*}
    and $i \geq 2$ as 
    \begin{equation*}
        m(\mathbf{x}, i) = \left(
            \begin{array}{ccc}
                x^1_1 & \dots & x^1_n \\
                \vdots & \ddots & \vdots \\ 
                x^{i-1}_1 & \dots & x^{i-1}_n \\ 
                x^{i-1}_1 & \dots & x^{i}_{n-1} \\ 
                \vdots & \ddots & \vdots \\ 
                x^{i-1}_1 & \dots & x^{d}_{n-1} \\ 
            \end{array}
        \right)
    \end{equation*}
    is called \emph{mask augmentation}. 
\end{definition}
Thus, the mask augemtation at $i \in [d]$ holds back any new incoming information beyond the $(i-1)^{th}$ coordinate. The full composition of augmentations applied to a sequence $\mathbf{x} \in S(\R^d, 2) $ prior to computing the signature of the embedded sequence is then defined as
\begin{equation*}
    \gamma_i = m_i \circ \psi \circ \psi \ . 
\end{equation*}


==> multi_asset_spot/level.tex <==
\begin{table}[h!]\centering\begin{tabular}{lllll}\toprule Model / Test metrics & $|\rho^x_h - \rho^x_g|_1$ & $|\kappa^x_h - \kappa^x_g|_1$ & $|s_h^x - s_g^x|_1$ & $|\Sigma_h^x - \Sigma_g^x|_1$ \\ \midrule Sig-Spline (Order 1)& $ 0.0001 \pm 0.0001$ & $ 0.0167 \pm 0.0053$ & $ 0.0031 \pm 0.0015$ & $ 0.0019 \pm 0.0003$ \\ \midrule Sig-Spline (Order 2)& $ 0.0001 \pm 0.0000$ & $ 0.0179 \pm 0.0071$ & $ 0.0039 \pm 0.0015$ & $ 0.0019 \pm 0.0002$ \\ \midrule Sig-Spline (Order 3)& $ 0.0001 \pm 0.0001$ & $ 0.0159 \pm 0.0046$ & $ 0.0028 \pm 0.0012$ & $ 0.0017 \pm 0.0003$ \\ \midrule Sig-Spline (Order 4)& $ 0.0001 \pm 0.0000$ & $ 0.0138 \pm 0.0052$ & $ 0.0028 \pm 0.0015$ & $ 0.0018 \pm 0.0004$ \\ \midrule Neural spline flow& $0.0001 \pm 0.0001$ & $0.0096 \pm 0.0060$ & $0.0046 \pm 0.0016$ & $0.0011 \pm 0.0008$ \\ \bottomrule \end{tabular}\caption{multi asset spot level}\end{table}

==> multi_asset_spot/level_decoded.tex <==
\begin{table}[h!]\centering\begin{tabular}{lllll}\toprule Model / Test metrics & $|\rho^x_h - \rho^x_g|_1$ & $|\kappa^x_h - \kappa^x_g|_1$ & $|s_h^x - s_g^x|_1$ & $|\Sigma_h^x - \Sigma_g^x|_1$ \\ \midrule Sig-Spline (Order 1)& $ 0.0514 \pm 0.0024$ & $ 12.3531 \pm 3.8606$ & $ 2.1035 \pm 0.2051$ & $ 0.0114 \pm 0.0005$ \\ \midrule Sig-Spline (Order 2)& $ 0.0512 \pm 0.0017$ & $ 12.1088 \pm 1.5706$ & $ 2.1740 \pm 0.2255$ & $ 0.0113 \pm 0.0005$ \\ \midrule Sig-Spline (Order 3)& $ 0.0512 \pm 0.0019$ & $ 12.1351 \pm 2.1431$ & $ 2.2561 \pm 0.2170$ & $ 0.0114 \pm 0.0006$ \\ \midrule Sig-Spline (Order 4)& $ 0.0509 \pm 0.0012$ & $ 11.6385 \pm 1.6616$ & $ 2.2019 \pm 0.2160$ & $ 0.0114 \pm 0.0005$ \\ \midrule Neural spline flow& $0.0526 \pm 0.0016$ & $8.9922 \pm 0.6928$ & $1.9180 \pm 0.0765$ & $0.0112 \pm 0.0003$ \\ \bottomrule \end{tabular}\caption{multi asset spot level}\end{table}
